LAMOL: LAnguage MOdeling for Lifelong Language Learning

Most research on lifelong learning applies to images or games, but not language. We present LAMOL, a simple yet effective method for lifelong language learning (LLL) based on language modeling. LAMOL replays pseudo-samples of previous tasks while requiring no extra memory or model capacity. Specifically, LAMOL is a language model that simultaneously learns to solve the tasks and generate training samples. When the model is trained for a new task, it generates pseudo-samples of previous tasks for training alongside data for the new task. The results show that LAMOL prevents catastrophic forgetting without any sign of intransigence and can perform five very different language tasks sequentially with only one model. Overall, LAMOL outperforms previous methods by a considerable margin and is only 2-3% worse than multitasking, which is usually considered the LLL upper bound. The source code is available at https://github.com/jojotenya/LAMOL.

==> figures/cmp_gen_size.tex <==
\begin{wrapfigure}{l}{0.5\textwidth}
  \includegraphics[width=\linewidth]{imgs/cmp_gen_size.png}
  \caption{Performance over after each epoch under five different sampling ratio and with or without task specific-specific tokens. In total, ten combinations are tested on the four tasks, WikiSQL, SST, QA-SRL, and WOZ.}
  \label{fig:cmp_gen_size}
\end{wrapfigure}


==> figures/five_tasks.tex <==
\begin{wrapfigure}{i}{0.5\textwidth}

  %\captionsetup{width=0.5\linewidth}
  \includegraphics[width=\linewidth]{imgs/five_tasks.png}
  
  \caption{Training progress of the five tasks. The graph records the performance of the model at each epoch of each tasks. The order of tasks in the progress follows: SQuAD, WikiSQL, SST, QA-SRL, and then WOZ.}
  \label{fig:five_tasks}
\end{wrapfigure}


==> tables/LM_format.tex <==
\begin{table}[t]
\centering
    \begin{tabu}{l||c|c|c|c|c|[2pt]c|c|c}
    \toprule
    Output & \multicolumn{2}{c|}{Context} & \multicolumn{2}{c|}{Question} & ANS & \multicolumn{2}{c|}{Answer} & EOS \\
    \midrule
    Input & GEN & \multicolumn{2}{c|}{Context} & \multicolumn{2}{c|[2pt]}{Question} & ANS & \multicolumn{2}{c}{Answer} \\
    \bottomrule
    \end{tabu}
    \caption{LM format}
\label{tab:LM_format}
\end{table}

==> tables/QA_format.tex <==
\begin{table}[t]
\centering
    \begin{tabu}{l|*{4}{|c}|[2pt]c|c|c}
    \toprule
    Output & IGN & \multicolumn{2}{c|}{$\dots$} & IGN & \multicolumn{2}{c|}{Answer} & EOS \\
    \midrule
    Input & \multicolumn{2}{c|}{Context} & \multicolumn{2}{c|[2pt]}{Question} & ANS & \multicolumn{2}{c}{Answer} \\
    \bottomrule
    \end{tabu}
    \caption{QA format}
\label{tab:QA_format}
\end{table}

==> tables/five_tasks_tmp.tex <==
\begin{table}[]
\centering
    \begin{tabular}{lccccccccc}
    \toprule
    {} &  finetune &   mas &  0.05 &  tag-0.05 &  real-0.05 &   0.2 &  tag-0.2 &  real-0.2 &  multitask \\
    \midrule
    squad1  &     35.75 & 40.05 & 55.65 &     56.33 &      64.70 & 58.22 &    61.87 &     68.68 &      76.93 \\
    wikisql &      1.21 &  1.45 & 50.38 &     59.57 &      65.06 & 64.13 &    64.40 &     66.99 &      72.71 \\
    sst     &     75.56 & 62.38 & 89.51 &     88.96 &      91.21 & 89.79 &    90.50 &     90.83 &      89.95 \\
    srl     &     59.68 & 58.09 & 67.78 &     67.07 &      67.11 & 68.27 &    69.49 &     69.08 &      69.98 \\
    woz.en  &     85.42 & 85.36 & 84.81 &     85.42 &      84.63 & 85.05 &    85.42 &     84.45 &      73.03 \\
    Ave.    &     51.52 & 49.46 & 69.63 &     71.47 &      74.54 & 73.09 &    74.33 &     76.01 &      76.52 \\
    \bottomrule
    \end{tabular}
    \caption{The result that different training manner test on each tasks' testing dataset after the last task has been trained. The boundaries of each task are clear in this set-up. For the column names, finetune, mas and multitask are corresponding to fine-tune, mas and multitask manner; 0.05 and 0.2 represent the percentage of previous tasks' (pseudo) data are generated for new tasks; "tag" means the manner assigns a specific tag for representing each task. "real" means keep true sample for new tasks.}
\label{tab:bound-model-to-tasks}
\end{table}

\begin{table}[]
    \centering
\begin{tabular}{lccccccccc}
\toprule
{} & finetune &     mas &    0.05 & tag-0.05 & real-0.05 &     0.2 & tag-0.2 & real-0.2 \\
\midrule
squad1  &        - &       - &       - &        - &         - &       - &       - &        - \\
wikisql &  -41.68\% & -49.95\% &  -8.61\% &   -8.61\% &    -4.61\% &  -7.24\% &  -8.05\% &   -3.36\% \\
sst     &  -86.63\% & -84.40\% & -23.07\% &  -18.14\% &   -10.22\% & -14.86\% & -13.65\% &   -6.93\% \\
srl     &  -28.95\% & -27.86\% & -22.32\% &  -21.39\% &   -12.21\% & -19.67\% & -14.43\% &   -8.82\% \\
woz.en  &  -53.32\% & -48.07\% & -27.83\% &  -26.95\% &   -16.10\% & -24.51\% & -19.59\% &  -10.91\% \\
\bottomrule
    \end{tabular}
    \caption{The result shows how much performance testing on SQuAD drops during training procedure for each manner. The boundaries of each task are clear. At the moment a task (excluding SQuAd itself) has been trained to converge, the model is used to test the SQuAd dataset. For the column names, finetune, mas and multitask are corresponding to fine-tune, mas and multitask manner; 0.05 and 0.2 represent the percentage of previous tasks' (pseudo) data are generated for new tasks; "tag" means the manner assigns a specific tag for representing each task. "real" means keep true sample for new tasks.}
    \label{tab:bound-squad-forget}
\end{table}

==> tables/text_cls_order1.tex <==
\begin{table}[t]
\centering
    \begin{tabular}{l*{4}{c}}
    \toprule
     & \footnotesize LAMOL_{Gen}^5 & \footnotesize LAMOL_{Task}^5 & \footnotesize LAMOL_{Gen}^{20} & \footnotesize LAMOL_{Task}^{20} \\
    \midrule
    Score & 72.2 & 76.5 & 77.4 & 77.0 \\
    \bottomrule
    \end{tabular}
    \caption{Summary of results on text classification tasks useing averaged EM score under different sample \% and tag usage against Order i in Table \ref{tab:text_cls}.}
\label{tab:text_cls_order1}
\end{table}
